Performant Synchronization in Geo-Distributed Databases

The deployment of databases across geographically distributed regions has become increasingly critical for ensuring data reliability and scalability. Recent studies indicate that distributed databases exhibit significantly higher latency than single-node databases, primarily due to consensus protocols maintaining data consistency across multiple nodes. We argue that synchronization cost constitutes the primary bottleneck for distributed databases, which is particularly pronounced in wide-area networks (WAN). Fortunately, we identify opportunities to optimize synchronization costs in real production environments: (1) network clustering phenomena, (2) triangle inequality violations in transmission, and (3) redundant data transfers. Based on these observations, we propose GeoCoCo, a synchronization acceleration framework for cross-region distributed databases. First, GeoCoCo presents a group rescheduling strategy that adapts to real-time network conditions to maximize WAN transmission efficiency. Second, GeoCoCo introduces a task-preserving data filtering method that reduces data volume transmitted over the WAN. Finally, GeoCoCo develops a consistency-guaranteed transmission framework integrating grouping and pruning. Extensive evaluations in both trace-driven simulations and real-world deployments demonstrate that GeoCoCo reduces synchronization cost-primarily by lowering WAN bandwidth usage-by up to 40.3%, and increases system throughput by up to 14.1% in GeoGauss.

==> Chapters/0_Abstract.tex <==


% Extensive evaluations in both trace-driven simulations and real-world deployments demonstrate that \name{} reduces synchronization cost by up to 40.3\%, and improves system throughput up to 14.1\% in GeoGauss, and scales efficiently to globally distributed datacenter clusters.
% Extensive evaluations in both trace-driven simulations and real-world deployments demonstrate that \name{} reduces synchronization cost by up to 40.3\%, improves system throughput by up to 14.1\% in GeoGauss, and scales efficiently to globally distributed datacenter clusters.


% The paper introduces \name, a high-performance collective communication framework designed for geo-distributed applications, addressing challenges like high latency, low bandwidth, and instability in Wide Area Networks (WANs). By optimizing collective communication operations (e.g., All-to-All, All-Reduce), the framework significantly improves transaction consistency in distributed databases and accelerates model convergence in distributed AI training. \name ensures efficient communication, reducing latency and bandwidth consumption, and provides a robust foundation for geo-distributed systems.

% Geographically distributed Database systems face critical performance bottlenecks due to WAN latency, limited bandwidth, and data redundancy. Common collective operations, such as All-to-All and AllReduce, amplify these challenges.
% We present \name{}, a general-purpose collective communication framework optimized for WAN environments. \name{} introduces hierarchical communication, latency violation-based grouping strategies, and lossless "white data" filtering.
% Experiments on both simulated environments and a real database system show that \name{} reduces All-to-All makespan by up to xx\%, improves throughput in GeoGauss, and scales to thousands of nodes with minimal performance overhead.

% 为了增强数据的可靠性与可扩展性，将数据库部署在跨地域的场景下成为了越来越重要的现实需求。
% 最近的研究表明分布式数据库的延迟要远远高于单机数据库，其原因是需要执行共识协议保持多个节点上的数据一致性。
% 我们argue同步代价是分布式数据库的主要bottle network, 这在跨域场景下尤为明显。
% 幸运的是，我们在实际的成产环境中发现了优化同步代价的机会，包括网络环境的聚集现象，和传输三角不等式，以及无用数据的传输。
% 基于这些观察，我们提出了\name{}，一个用于跨域分布式数据库中的聚合通讯加速框架。
% \name{}首先提出了一个根据实时网络环境的分组重排策略以充分释放广域网的传输上限。
% 其次，\name{}提出了一种保持任务正确的数据剪枝方法以减少广域网上传输的数据量。
% 最后，\name{}提出了一个基于分组和剪枝的保证一致性的传输框架。
% Extensive evaluations in both trace-driven simulations and real-world deployments demonstrate that \name{} reduces All-to-All completion time by up to xxx\%, improves system throughput in GeoGauss, and scales efficiently to globally distributed datacenter clusters.

% Geo-distributed database systems face fundamental performance bottlenecks in wide-area networks (WANs), including high latency, limited bandwidth, and excessive data redundancy.
% Common collective operations, such as All-to-All and AllReduce, further exacerbate these challenges due to their intensive communication demands.
% We present \name{}, a general-purpose collective communication framework optimized for WAN environments. \name{} introduces hierarchical communication, latency violation-based grouping strategies, and lossless "white data" filtering.
% Extensive evaluations in both trace-driven simulations and real-world deployments demonstrate that \name{} reduces All-to-All completion time by up to xxx\%, improves system throughput in GeoGauss, and scales efficiently to globally distributed datacenter clusters.



  % A clear and well-documented \LaTeX\ document is presented as an
  % article formatted for publication by ACM in a conference proceedings
  % or journal publication. Based on the ``acmart'' document class, this
  % article presents and explains many of the common variations, as well
  % as many of the formatting elements an author may use in the
  % preparation of the documentation of their work.


==> Chapters/7_DISCUSSION.tex <==

    % \subsection{Payload Size}
    \subsection{Number of Group}

    \subsection{The bottleneck }

    
    \subsection{Cases for bandwidth or latency unlimited}
    In wide area networks, it is generally recognized that both bandwidth and latency will be limited, which has an impact on the transmission effect. However, for the sake of rigor, we still separately discuss the adaptability of our framework when bandwidth or latency is not restricted, and quantitatively test its transmission performance.

    % to show the result of 2 s.
    % 这里可以放一些定量的理论推导进行讨论。当带宽或者时延不受限的时候的理论收益和实际结果。


    
    \subsection{\name~ in big cluster}

    
    \subsection{Performance Under Failures}

==> Chapters/Future_work.tex <==


While \name{} has demonstrated substantial benefits in optimizing synchronization within geo-distributed databases, its underlying principles—such as hierarchical communication and structure-aware grouping—can be generalized to other distributed domains.
A natural extension of this work is applying \name{} to distributed machine learning and federated training settings. In these environments, a central server often needs to aggregate updates from a large number of geographically dispersed edge nodes~\cite{deng2009imagenet, zhang2021survey, asad2021thf, hellings2021byshard, hsieh2017gaia, llm_pruner}.
By incorporating \name{}’s latency-aware grouping and intermediate aggregation, we anticipate improvements in global model synchronization speed and communication efficiency~\cite{fei2021efficient, jiang2020unified}.
Looking ahead, we plan to explore this direction by integrating \name{} into real-world federated learning frameworks, enabling scalable, WAN-optimized training across thousands of heterogeneous nodes~\cite{wu2020cloud,laghari2021review}.


% While we have applied \name~ to geographically distributed collective communication scenarios such as All-to-All and All-Reduce, its design principles and optimization strategies could be beneficial in a broader range of distributed systems. For instance, federated learning systems often require aggregating updates from a large number of edge devices spread across diverse geographic regions~\cite{zhang2021survey,asad2021thf}. These systems typically face challenges such as high latency, uneven bandwidth distribution, and limited computational resources at edge nodes. Applying \name~’s hierarchical communication model and dynamic path selection to federated learning could help mitigate latency bottlenecks and improve global model synchronization, particularly in large-scale deployments with thousands of edge devices.
% Another potential future work is integrating \name~ into hybrid cloud-edge architectures, where communication between cloud data centers and edge nodes involves complex multi-hop topologies~\cite{wu2020cloud}. By leveraging \name~’s group-based strategies and “white data” filtering techniques, the framework could enhance the efficiency of data exchange for use cases such as IoT data aggregation, video streaming optimization, and cross-region disaster recovery~\cite{wu2020cloud,laghari2021review}. Extending \name~ to these emerging scenarios offers an exciting opportunity to improve communication efficiency and scalability across diverse distributed systems.

==> Chapters/PERFORMANCE_EVALUATION.tex <==
\subsection{Implementation and testbed.}
\textbf{Trace-based Simulation.}In our multi-round performance evaluation, we comprehensively considered the impact of different network topologies and load distributions on the algorithm’s performance. End-to-end performance experiments adopted a trace-based approach, utilizing the TC (Traffic Control) tool~\cite{tc} to simulate real-world wide-area network (WAN) latency datasets, enabling precise emulation of communication delays in WAN environments.

\noindent  \textbf{Distributed Multi-Master Database Implementation.} 
We integrated the implementation of \name into GeoGauss. GeoGauss is a high-performance database system designed specifically for geo-distributed environments, providing optimized transaction processing and distributed storage capabilities. To validate the communication optimization of \name on GeoGauss~\cite{zhou2023geogauss}, 
we used the standard YCSB benchmark~\cite{cooper2010benchmarking} tool 
to evaluate the framework’s performance within the GeoGauss system. The testing was conducted in a cloud computing environment composed of multiple physical machines, each equipped with 12-core vCPUs and 48 GiB memory.


\noindent  \textbf{Distributed Training Simulation.} 
We also integrated the framework into modified versions of 
Astra-Sim~\cite{rashidi2020astra,won2023astra} and 
NS-3 simulators~\cite{riley2010ns,henderson2008network,ns3}. 
Astra-Sim is a high-performance simulation platform specifically designed for distributed deep learning tasks, supporting end-to-end deep learning communication modeling. NS-3, on the other hand, is used for precise modeling of underlying network transmission characteristics. Both tools are widely adopted in academic research and industrial testing scenarios~\cite{sharma2024gpu,shen2023mars,zhang2024poster,rashidi2020scalable}.
By combining the two, we were able to simulate and analyze network transmission behaviors in large-scale distributed training tasks, particularly focusing on the communication overhead of gradient aggregation and parameter synchronization. In our experiments, we simulated a distributed environment comprising thousands of nodes, each equipped with high-performance GPUs, to comprehensively evaluate the performance optimization of \name in distributed training.

\noindent \textbf{Results.}The experimental results demonstrate that \name significantly reduces communication latency and improves throughput in distributed multi-master database environments. Furthermore, \name effectively shortens training time in geo-distributed training tasks. Overall, \name has proven its versatility and efficiency, offering an effective solution for communication optimization in WAN and distributed computing environments.


\subsection{Single-Round Result}
\textbf{Single-Round on Dynamic Path Selection.}
We first validate the optimization effect of the dynamic path selection algorithm on the Makespan of each round of All-to-All communication under fluctuating high-latency and low-bandwidth conditions. The experiment utilizes real wide-area network latency traces from the 
dataset "Wonder Network"~\cite{wondernetwork2024}, 
while bandwidth values are derived from measurements on actual paths and subjected to random fluctuations within a predefined range to simulate dynamic network environments. To enable quantitative evaluation, we generate load data that mimics real-world transmission scenarios.
We compare the following three schemes:
1.	Origin: The original direct transmission scheme without grouping or path optimization.
2.	Optimal: The theoretical optimal Makespan obtained through post-hoc analysis of all latency and bandwidth combinations for the given load.
3.	\name: The proposed dynamic path selection scheme.

\begin{figure}
    \centering
    \includegraphics[width=1\linewidth]{figure/fig-cdf-result-after.pdf}
    % \caption{CDF Distribution of Makespan in 1000 Single-Round All-to-All Communications.}
    \caption{CDF Distribution of Single-Round Makespan.}
    \label{fig:cdf}
\end{figure}

\begin{figure}[t!]
    \centering
    \hspace*{-0.3cm}
    \subfigure{ \label{fig: heat-no-group}
        \begin{minipage}[b]{0.5\linewidth}
            \includegraphics[width=\linewidth]{figure/fig-heat-nogroup.pdf}
        \end{minipage}
    }
    \hspace*{-0.3cm}
    \subfigure{ \label{fig: heat-our}
        \begin{minipage}[b]{0.5\linewidth}
            \includegraphics[width=\linewidth]{figure/fig-heat-our.pdf}
        \end{minipage}
    \caption{(a) Heatmap of Communication Frequency Without Transmission Grouping (Baseline). (b) Heatmap of Communication Frequency with Transmission Grouping Using \name.}
    \label{fig: heatmaps}
\end{figure}


The figure~\ref{fig:cdf} presents the cumulative distribution function (CDF) of Makespan across 1000 single-round All-to-All communication experiments. The main plot illustrates the overall distribution of completion times, while the inset plot zooms in on the [0.4, 1.0] range to highlight finer details.
\name~(Grouping, dark blue) employs a dynamic path optimization method through grouping, achieving completion times that closely approach the theoretical optimal value~(Low Bound, light blue). This demonstrates a significant improvement in the performance of the Makespan distribution. Compared to the direct cross-domain transmission scheme~(Origin, green), \name achieves shorter completion times in the majority of cases, reflecting its effective optimization capabilities.
Additionally, \name reduces the longest Makespan by 6.89\% compared to the original scheme, showcasing its ability to optimize under extreme conditions. Furthermore, \name reduces the 99th percentile latency by 26\%, highlighting its effectiveness in mitigating tail latency and improving performance reliability.
% \vspace{-0.4cm}



Heatmap of communication frequency distribution
(in Figure~\ref{fig: heatmaps}) based on the statistics collected after multiple rounds of grouped communication. Subfigure (a) illustrates the communication frequency distribution under the original scheme without grouping, while subfigure (b) shows the distribution after applying the grouping scheme. The color intensity in the heatmap reflects the normalized communication frequency, with darker shades indicating higher frequencies.
Compared to the original scheme, where each round of All-to-All transmission requires two fully connected transmissions, the \name reduces the usage of long-latency paths through optimized grouping strategies, resulting in a significant 63.35\% reduction in overall communication frequency. More importantly, this optimization achieves lower communication frequency without compromising performance or degrading single-round completion times, further demonstrating the effectiveness of ~\name
~in improving communication efficiency while maintaining performance reliability.



\vspace{0.3ex} \noindent \textbf{Single-Round on Dynamic Path Selection + Data Aggregation.}

==> Chapters/other.tex <==
% \section{Modifications}

% Modifying the template --- including but not limited to: adjusting
% margins, typeface sizes, line spacing, paragraph and list definitions,
% and the use of the \verb|\vspace| command to manually adjust the
% vertical spacing between elements of your work --- is not allowed.

% % {\bfseries Your document will be returned to you for revision if
% %   modifications are discovered.}

% \section{Typefaces}

% The ``\verb|acmart|'' document class requires the use of the
% ``Libertine'' typeface family. Your \TeX\ installation should include
% this set of packages. Please do not substitute other typefaces. The
% ``\verb|lmodern|'' and ``\verb|ltimes|'' packages should not be used,
% as they will override the built-in typeface families.

% \section{Title Information}

% The title of your work should use capital letters appropriately -
% \url{https://capitalizemytitle.com/} has useful rules for
% capitalization. Use the {\verb|title|} command to define the title of
% your work. If your work has a subtitle, define it with the
% {\verb|subtitle|} command.  Do not insert line breaks in your title.

% If your title is lengthy, you must define a short version to be used
% in the page headers, to prevent overlapping text. The \verb|title|
% command has a ``short title'' parameter:
% \begin{verbatim}
%   \title[short title]{full title}
% \end{verbatim}

% \section{Authors and Affiliations}

% Each author must be defined separately for accurate metadata
% identification.  As an exception, multiple authors may share one
% affiliation. Authors' names should not be abbreviated; use full first
% names wherever possible. Include authors' e-mail addresses whenever
% possible.

% Grouping authors' names or e-mail addresses, or providing an ``e-mail
% alias,'' as shown below, is not acceptable:
% \begin{verbatim}
%   \author{Brooke Aster, David Mehldau}
%   \email{dave,judy,steve@university.edu}
%   \email{firstname.lastname@phillips.org}
% \end{verbatim}

% The \verb|authornote| and \verb|authornotemark| commands allow a note
% to apply to multiple authors --- for example, if the first two authors
% of an article contributed equally to the work.

% If your author list is lengthy, you must define a shortened version of
% the list of authors to be used in the page headers, to prevent
% overlapping text. The following command should be placed just after
% the last \verb|\author{}| definition:
% \begin{verbatim}
%   \renewcommand{\shortauthors}{McCartney, et al.}
% \end{verbatim}
% Omitting this command will force the use of a concatenated list of all
% of the authors' names, which may result in overlapping text in the
% page headers.

% The article template's documentation, available at
% \url{https://www.acm.org/publications/proceedings-template}, has a
% complete explanation of these commands and tips for their effective
% use.

% Note that authors' addresses are mandatory for journal articles.

% \section{Rights Information}

% Authors of any work published by ACM will need to complete a rights
% form. Depending on the kind of work, and the rights management choice
% made by the author, this may be copyright transfer, permission,
% license, or an OA (open access) agreement.

% Regardless of the rights management choice, the author will receive a
% copy of the completed rights form once it has been submitted. This
% form contains \LaTeX\ commands that must be copied into the source
% document. When the document source is compiled, these commands and
% their parameters add formatted text to several areas of the final
% document:
% \begin{itemize}
% \item the ``ACM Reference Format'' text on the first page.
% \item the ``rights management'' text on the first page.
% \item the conference information in the page header(s).
% \end{itemize}

% Rights information is unique to the work; if you are preparing several
% works for an event, make sure to use the correct set of commands with
% each of the works.

% The ACM Reference Format text is required for all articles over one
% page in length, and is optional for one-page articles (abstracts).

% \section{CCS Concepts and User-Defined Keywords}

% Two elements of the ``acmart'' document class provide powerful
% taxonomic tools for you to help readers find your work in an online
% search.

% The ACM Computing Classification System ---
% \url{https://www.acm.org/publications/class-2012} --- is a set of
% classifiers and concepts that describe the computing
% discipline. Authors can select entries from this classification
% system, via \url{https://dl.acm.org/ccs/ccs.cfm}, and generate the
% commands to be included in the \LaTeX\ source.

% User-defined keywords are a comma-separated list of words and phrases
% of the authors' choosing, providing a more flexible way of describing
% the research being presented.

% CCS concepts and user-defined keywords are required for for all
% articles over two pages in length, and are optional for one- and
% two-page articles (or abstracts).

% \section{Sectioning Commands}

% Your work should use standard \LaTeX\ sectioning commands:
% \verb|section|, \verb|subsection|, \verb|subsubsection|, and
% \verb|paragraph|. They should be numbered; do not remove the numbering
% from the commands.

% Simulating a sectioning command by setting the first word or words of
% a paragraph in boldface or italicized text is {\bfseries not allowed.}

% \section{Tables}

% The ``\verb|acmart|'' document class includes the ``\verb|booktabs|''
% package --- \url{https://ctan.org/pkg/booktabs} --- for preparing
% high-quality tables.

% Table captions are placed {\itshape above} the table.

% Because tables cannot be split across pages, the best placement for
% them is typically the top of the page nearest their initial cite.  To
% ensure this proper ``floating'' placement of tables, use the
% environment \textbf{table} to enclose the table's contents and the
% table caption.  The contents of the table itself must go in the
% \textbf{tabular} environment, to be aligned properly in rows and
% columns, with the desired horizontal and vertical rules.  Again,
% detailed instructions on \textbf{tabular} material are found in the
% \textit{\LaTeX\ User's Guide}.

% Immediately following this sentence is the point at which
% Table~\ref{tab:freq} is included in the input file; compare the
% placement of the table here with the table in the printed output of
% this document.

% \begin{table}
%   \caption{Frequency of Special Characters}
%   \label{tab:freq}
%   \begin{tabular}{ccl}
%     \toprule
%     Non-English or Math&Frequency&Comments\\
%     \midrule
%     \O & 1 in 1,000& For Swedish names\\
%     $\pi$ & 1 in 5& Common in math\\
%     \$ & 4 in 5 & Used in business\\
%     $\Psi^2_1$ & 1 in 40,000& Unexplained usage\\
%   \bottomrule
% \end{tabular}
% \end{table}

% To set a wider table, which takes up the whole width of the page's
% live area, use the environment \textbf{table*} to enclose the table's
% contents and the table caption.  As with a single-column table, this
% wide table will ``float'' to a location deemed more
% desirable. Immediately following this sentence is the point at which
% Table~\ref{tab:commands} is included in the input file; again, it is
% instructive to compare the placement of the table here with the table
% in the printed output of this document.

% \begin{table*}
%   \caption{Some Typical Commands}
%   \label{tab:commands}
%   \begin{tabular}{ccl}
%     \toprule
%     Command &A Number & Comments\\
%     \midrule
%     \texttt{{\char'134}author} & 100& Author \\
%     \texttt{{\char'134}table}& 300 & For tables\\
%     \texttt{{\char'134}table*}& 400& For wider tables\\
%     \bottomrule
%   \end{tabular}
% \end{table*}

% Always use midrule to separate table header rows from data rows, and
% use it only for this purpose. This enables assistive technologies to
% recognise table headers and support their users in navigating tables
% more easily.

% \section{Math Equations}
% You may want to display math equations in three distinct styles:
% inline, numbered or non-numbered display.  Each of the three are
% discussed in the next sections.

% \subsection{Inline (In-text) Equations}
% A formula that appears in the running text is called an inline or
% in-text formula.  It is produced by the \textbf{math} environment,
% which can be invoked with the usual
% \texttt{{\char'134}begin\,\ldots{\char'134}end} construction or with
% the short form \texttt{\$\,\ldots\$}. You can use any of the symbols
% and structures, from $\alpha$ to $\omega$, available in
% \LaTeX~\cite{Lamport:LaTeX}; this section will simply show a few
% examples of in-text equations in context. Notice how this equation:
% \begin{math}
%   \lim_{n\rightarrow \infty}x=0
% \end{math},
% set here in in-line math style, looks slightly different when
% set in display style.  (See next section).

% \subsection{Display Equations}
% A numbered display equation---one set off by vertical space from the
% text and centered horizontally---is produced by the \textbf{equation}
% environment. An unnumbered display equation is produced by the
% \textbf{displaymath} environment.

% Again, in either environment, you can use any of the symbols and
% structures available in \LaTeX\@; this section will just give a couple
% of examples of display equations in context.  First, consider the
% equation, shown as an inline equation above:
% \begin{equation}
%   \lim_{n\rightarrow \infty}x=0
% \end{equation}
% Notice how it is formatted somewhat differently in
% the \textbf{displaymath}
% environment.  Now, we'll enter an unnumbered equation:
% \begin{displaymath}
%   \sum_{i=0}^{\infty} x + 1
% \end{displaymath}
% and follow it with another numbered equation:
% \begin{equation}
%   \sum_{i=0}^{\infty}x_i=\int_{0}^{\pi+2} f
% \end{equation}
% just to demonstrate \LaTeX's able handling of numbering.

% \section{Figures}

% The ``\verb|figure|'' environment should be used for figures. One or
% more images can be placed within a figure. If your figure contains
% third-party material, you must clearly identify it as such, as shown
% in the example below.
% \begin{figure}[h]
%   \centering
%   \includegraphics[width=\linewidth]{sample-franklin}
%   \caption{1907 Franklin Model D roadster. Photograph by Harris \&
%     Ewing, Inc. [Public domain], via Wikimedia
%     Commons. (\url{https://goo.gl/VLCRBB}).}
%   \Description{A woman and a girl in white dresses sit in an open car.}
% \end{figure}

% Your figures should contain a caption which describes the figure to
% the reader.



% \subsection{The ``Teaser Figure''}

% A ``teaser figure'' is an image, or set of images in one figure, that
% are placed after all author and affiliation information, and before
% the body of the article, spanning the page. If you wish to have such a
% figure in your article, place the command immediately before the
% \verb|\maketitle| command:
% \begin{verbatim}
%   \begin{teaserfigure}
%     \includegraphics[width=\textwidth]{sampleteaser}
%     \caption{figure caption}
%     \Description{figure description}
%   \end{teaserfigure}
% \end{verbatim}

% \section{Citations and Bibliographies}

% The use of \BibTeX\ for the preparation and formatting of one's
% references is strongly recommended. Authors' names should be complete
% --- use full first names (``Donald E. Knuth'') not initials
% (``D. E. Knuth'') --- and the salient identifying features of a
% reference should be included: title, year, volume, number, pages,
% article DOI, etc.

% The bibliography is included in your source document with these two
% commands, placed just before the \verb|\end{document}| command:
% \begin{verbatim}
%   \bibliographystyle{ACM-Reference-Format}
%   \bibliography{bibfile}
% \end{verbatim}
% where ``\verb|bibfile|'' is the name, without the ``\verb|.bib|''
% suffix, of the \BibTeX\ file.

% Citations and references are numbered by default. A small number of
% ACM publications have citations and references formatted in the
% ``author year'' style; for these exceptions, please include this
% command in the {\bfseries preamble} (before the command
% ``\verb|\begin{document}|'') of your \LaTeX\ source:
% \begin{verbatim}
%   \citestyle{acmauthoryear}
% \end{verbatim}


%   Some examples.  A paginated journal article \cite{Abril07}, an
%   enumerated journal article \cite{Cohen07}, a reference to an entire
%   issue \cite{JCohen96}, a monograph (whole book) \cite{Kosiur01}, a
%   monograph/whole book in a series (see 2a in spec. document)
%   \cite{Harel79}, a divisible-book such as an anthology or compilation
%   \cite{Editor00} followed by the same example, however we only output
%   the series if the volume number is given \cite{Editor00a} (so
%   Editor00a's series should NOT be present since it has no vol. no.),
%   a chapter in a divisible book \cite{Spector90}, a chapter in a
%   divisible book in a series \cite{Douglass98}, a multi-volume work as
%   book \cite{Knuth97}, a couple of articles in a proceedings (of a
%   conference, symposium, workshop for example) (paginated proceedings
%   article) \cite{Andler79, Hagerup1993}, a proceedings article with
%   all possible elements \cite{Smith10}, an example of an enumerated
%   proceedings article \cite{VanGundy07}, an informally published work
%   \cite{Harel78}, a couple of preprints \cite{Bornmann2019,
%     AnzarootPBM14}, a doctoral dissertation \cite{Clarkson85}, a
%   master's thesis: \cite{anisi03}, an online document / world wide web
%   resource \cite{Thornburg01, Ablamowicz07, Poker06}, a video game
%   (Case 1) \cite{Obama08} and (Case 2) \cite{Novak03} and \cite{Lee05}
%   and (Case 3) a patent \cite{JoeScientist001}, work accepted for
%   publication \cite{rous08}, 'YYYYb'-test for prolific author
%   \cite{SaeediMEJ10} and \cite{SaeediJETC10}. Other cites might
%   contain 'duplicate' DOI and URLs (some SIAM articles)
%   \cite{Kirschmer:2010:AEI:1958016.1958018}. Boris / Barbara Beeton:
%   multi-volume works as books \cite{MR781536} and \cite{MR781537}. A
%   couple of citations with DOIs:
%   \cite{2004:ITE:1009386.1010128,Kirschmer:2010:AEI:1958016.1958018}. Online
%   citations: \cite{TUGInstmem, Thornburg01, CTANacmart}.
%   Artifacts: \cite{R} and \cite{UMassCitations}.

% \section{Acknowledgments}

% Identification of funding sources and other support, and thanks to
% individuals and groups that assisted in the research and the
% preparation of the work should be included in an acknowledgment
% section, which is placed just before the reference section in your
% document.

% This section has a special environment:
% \begin{verbatim}
%   \begin{acks}
%   ...
%   \end{acks}
% \end{verbatim}
% so that the information contained therein can be more easily collected
% during the article metadata extraction phase, and to ensure
% consistency in the spelling of the section heading.

% Authors should not prepare this section as a numbered or unnumbered {\verb|\section|}; please use the ``{\verb|acks|}'' environment.

% \section{Appendices}

% If your work needs an appendix, add it before the
% ``\verb|\end{document}|'' command at the conclusion of your source
% document.

% Start the appendix with the ``\verb|appendix|'' command:
% \begin{verbatim}
%   \appendix
% \end{verbatim}
% and note that in the appendix, sections are lettered, not
% numbered. This document has two appendices, demonstrating the section
% and subsection identification method.

% \section{Multi-language papers}

% Papers may be written in languages other than English or include
% titles, subtitles, keywords and abstracts in different languages (as a
% rule, a paper in a language other than English should include an
% English title and an English abstract).  Use \verb|language=...| for
% every language used in the paper.  The last language indicated is the
% main language of the paper.  For example, a French paper with
% additional titles and abstracts in English and German may start with
% the following command
% \begin{verbatim}
% \documentclass[sigconf, language=english, language=german,
%                language=french]{acmart}
% \end{verbatim}

% The title, subtitle, keywords and abstract will be typeset in the main
% language of the paper.  The commands \verb|\translatedXXX|, \verb|XXX|
% begin title, subtitle and keywords, can be used to set these elements
% in the other languages.  The environment \verb|translatedabstract| is
% used to set the translation of the abstract.  These commands and
% environment have a mandatory first argument: the language of the
% second argument.  See \verb|sample-sigconf-i13n.tex| file for examples
% of their usage.

% \section{SIGCHI Extended Abstracts}

% The ``\verb|sigchi-a|'' template style (available only in \LaTeX\ and
% not in Word) produces a landscape-orientation formatted article, with
% a wide left margin. Three environments are available for use with the
% ``\verb|sigchi-a|'' template style, and produce formatted output in
% the margin:
% \begin{description}
% \item[\texttt{sidebar}:]  Place formatted text in the margin.
% \item[\texttt{marginfigure}:] Place a figure in the margin.
% \item[\texttt{margintable}:] Place a table in the margin.
% \end{description}
